Role of Fluid Forces and Depletion Interactions in Directing Assembly of Aqueous Gold Nanorods on Hydrophobic Surfaces

The interaction between macroscopic fluid flow and nanoscale forces has resulted in the formation of long-range assemblies through evaporation-induced self-assembly. Anisotropic gold nanorods (AuNR) can form disordered, smectic, or vertically ordered long-range structures, but controlling their assembly remains a challenge and requires a deeper understanding of fundamental interaction mechanisms. In this work, we established a correlation between the $in~situ$ drying profiles, measured using an optical tensiometer, and deposit pattern, imaged $ex~situ$ using electron microscopy. Increasing particle concentration induced a transition from coffee-ring to uniform deposition at the microscale, while nanoscale structures shifted from isotropic/smectic to vertically aligned crystalline AuNRs. The interplay of capillary and Marangoni flow influences assembly at both macro and nanoscales, with the deposition process and nanoparticle ordering being highly sensitive to interparticle and nanoparticle-substrate interactions. By systematically studying key parameters, we aim to develop a comprehensive framework for the rational design and fabrication of nanomaterials with precisely controlled structure and properties.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
